Deep Prototypical-Parts Ease Morphological Kidney Stone Identification and are Competitively Robust to Photometric Perturbations

Identifying the type of kidney stones can allow urologists to determine their cause of formation, improving the prescription of appropriate treatments to diminish future relapses. Currently, the associated ex-vivo diagnosis (known as Morpho-constitutional Analysis, MCA) is time-consuming, expensive and requires a great deal of experience, as it requires a visual analysis component that is highly operator dependant. Recently, machine learning methods have been developed for in-vivo endoscopic stone recognition. Deep Learning (DL) based methods outperform non-DL methods in terms of accuracy but lack explainability. Despite this trade-off, when it comes to making high-stakes decisions, it's important to prioritize understandable Computer-Aided Diagnosis (CADx) that suggests a course of action based on reasonable evidence, rather than a model prescribing a course of action. In this proposal, we learn Prototypical Parts (PPs) per kidney stone subtype, which are used by the DL model to generate an output classification. Using PPs in the classification task enables case-based reasoning explanations for such output, thus making the model interpretable. In addition, we modify global visual characteristics to describe their relevance to the PPs and the sensitivity of our model's performance. With this, we provide explanations with additional information at the sample, class and model levels in contrast to previous works. Although our implementation's average accuracy is lower than state-of-the-art (SOTA) non-interpretable DL models by 1.5 %, our models perform 2.8% better on perturbed images with a lower standard deviation, without adversarial training. Thus, Learning PPs has the potential to create more robust DL models.

==> tables/Backbone_vs_PPs.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Comparison of ProtoPNet using different CNN architectures as the feature extractor against the pure finetuned CNN, with Data Augmentation (DA) and without Data Augmentation (NoDA)}
\label{Backbone_vs_PPs}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccccc}
\multirow{2}{*}{} & \multicolumn{2}{c}{DenseNet201} & \multicolumn{2}{c}{ResNet50} & \multicolumn{2}{c}{VGG16} \\
     & CNN    & PPs    & CNN    & PPs    & CNN    & PPs    \\ \hline
NoDA & 79.2\% & 84.1\% & 76.0\% & 83.1\% & 85.0\% & 76.9\% \\
DA   & 89.4\% & 85.5\% & 85.0\% & 85.9\% & 84.0\% & 81.0\%
\end{tabular}%
}
\end{table}

==> tables/Deletion_Boxplots_example.tex <==
\begin{figure}[ht] 
    \centering
    \includegraphics[width=1.0\linewidth]{imgs/deletion_ProtoPNet_vs_backbone_DenseNet201_long.pdf}
    \caption{\small{
    %Deletion scores per class comparing ProtoPNet heatmaps (in blue) against Grad-CAMs from its backbone (in orange). 
    Comparison of "deletion" scores by class of the heat maps obtained from a ProtoPnet, against those from GradCAM of a CNN. Both the ProtoPNet backbone and the separately trained CNN are a DenseNet201 convolutional architecture.
    In this case, ProtoPNet uses 3 prototypical parts per class and both networks are trained with data augmentation as described in section  \ref{Implementation_Details}. 
    It is observed, \textit{deletion} average ProtoPNet scores outperform GradCAMs, for three classes (WW, BRU, CYS). ProtoPNet "deletion" scores also present a reduced variability than the results presented by GradCAM, hence a more consistent behavior when generating .
    Classes WW, WD, AU, STR, BRU and CYS are described in section \ref{Kidney_stone_dataset}.
    %The classes observed are WW (Whewellite, type Ia), WD (Weddellite, type IIa), AU (Acide Urique, type IIIa), STR (Struvite, type IVc), BRU (Brushite, type IVd), CYS (Cystine, type Va).
    Image best seen in color.
    }}
    \label{fig:umaps}
\end{figure}

==> tables/Descriptors_example1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{}
\label{Descriptors_example1}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccc}
\multicolumn{3}{c}{Highest activated Prototypical-Part: 13th}                                                                                          \\ \hline
Descriptor & \begin{tabular}[c]{@{}c@{}}Local\\      Activation \%\end{tabular} & \begin{tabular}[c]{@{}c@{}}Global \\      Activation \%\end{tabular} \\ \hline
Hue        & 62.2\% & 33.6\% \\
Texture    & 60.7\% & 31.4\% \\
Contrast   & 57.6\% & 24.7\% \\
Shape      & 57.3\% & 23.5\% \\
Brightness & 49.7\% & 15.3\% \\
Saturation & 29.9\% & 15.0\% \\ \hline
Avg        & 52.9\% & 23.9\%
\end{tabular}%
}
\end{table}

==> tables/cvpr22_simpleTable.tex <==
\begin{table*}[]
\centering
\caption{\small{Weighted average metrics comparison for section, surface, and mixed patches. ProtoPNet with VGG19 with batch normalization as the backbone (PPN-VGG19bn). VGG 19-layer model, configuration `E', with batch normalization (VGG19bn).
}}
\label{tab:my-table}
\scalebox{0.88}{\begin{tabular}{@{}ccccccccccccc@{}}
\toprule
\multirow{2}{*}{Model} & \multicolumn{3}{c}{Accuracy} & \multicolumn{3}{c}{Precision} & \multicolumn{3}{c}{Recall} & \multicolumn{3}{c}{F1 score} \\ \cmidrule(l){2-13} 
                       & Surface  & Section  & Mixed  & Surface   & Section  & Mixed  & Surface  & Section & Mixed & Surface  & Section  & Mixed  \\ \midrule
PPN-VGG19bn            & 0.98     & 0.99     & 0.97   & 0.98      & 0.99     & 0.97   &
 0.98     & 0.99    & 0.97  & 0.98     & 0.99     & 0.97   \\
VGG19bn                & 0.99     & 1.00     & 1.00   & 0.99      & 1.00     & 1.00   & 0.99     & 1.00    & 1.00  & 0.99     & 1.00     & 1.00   \\
AlexNet                & 0.96     & 0.97     & 0.97   & 0.96      & 0.97     & 0.97   & 0.96     & 0.97    & 0.97  & 0.96     & 0.97     & 0.97   \\ \bottomrule
\end{tabular}
}
\end{table*}

==> tables/table_Descriptors_example.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{}
\label{table_Descriptors}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccc}
\multicolumn{4}{c}{PPs 13th}                                             \\ \hline
\multicolumn{2}{c}{Local Analysis} & \multicolumn{2}{c}{Global Analysis} \\ \hline
Descriptor & \begin{tabular}[c]{@{}c@{}}Local \\      Act. \%\end{tabular} & Descriptor & \begin{tabular}[c]{@{}c@{}}Global \\      Act. \%\end{tabular} \\ \hline
\textbf{Hue}    & \textbf{62\%}    & \textbf{Hue}     & \textbf{34\%}    \\
Texture         & 61\%             & Texture          & 31\%             \\
Contrast        & 58\%             & Contrast         & 25\%             \\
Shape           & 57\%             & Shape            & 24\%             \\
Brightness      & 50\%             & Brightness       & 15\%             \\
Saturation      & 30\%             & Saturation       & 15\%             \\ \hline
Avg             & 53\%             & Avg              & 24\%            
\end{tabular}%
}
\end{table}

==> tables/table_explanation_example_correctWD.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{}
\label{tab:my-table}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccc}
\multicolumn{3}{c}{Highest Prototipical-Part} \\ \hline
\multirow{3}{*}{Descriptor} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Local \\      Activation \%\end{tabular}} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Global\\      Activation\end{tabular}} \\
                 &              &             \\
                 &              &             \\ \hline
Contrast         & 65.7\%       & 51.8\%      \\
Hue              & 64.1\%       & 51.6\%      \\
Texture          & 54.7\%       & 29.1\%      \\
Shape            & 46.6\%       & 31.5\%      \\
Saturation       & 44.8\%       & 37.3\%      \\
Brightness       & 0.7\%        & 19.1\%      \\ \hline
Avg.             & 46.1\%       & 36.7\%     
\end{tabular}%
}
\end{table}
